Interactive Lab Notebooks for Robotics Researchers

Interactive notebooks, such as Jupyter, have revolutionized the field of data science by providing an integrated environment for data, code, and documentation. However, their adoption by robotics researchers and model developers has been limited. This study investigates the logging and record-keeping practices of robotics researchers, drawing parallels to the pre-interactive notebook era of data science. Through interviews with robotics researchers, we identified the reliance on diverse and often incompatible tools for managing experimental data, leading to challenges in reproducibility and data traceability. Our findings reveal that robotics researchers can benefit from a specialized version of interactive notebooks that supports comprehensive data entry, continuous context capture, and agile data staging. We propose extending interactive notebooks to better serve the needs of robotics researchers by integrating features akin to traditional lab notebooks. This adaptation aims to enhance the organization, analysis, and reproducibility of experimental data in robotics, fostering a more streamlined and efficient research workflow.

==> stateofplay.tex <==
% Section 2

% Template: SW Eng standard tool. Differences in the MML. List of failings of tool. Potential solutions in the data world. Need for integration of worldviews/tools.

% Pipeline Dev. State of play: IDEs and version control. Talk about how data changes the story for SW eng. List k top needs that these donot fulfill. Then bring up Jupyter and Tableau, but point out how they don't do a good job with code.
